Remote Credential Management with Mutual Attestation for Trusted Execution Environments

Trusted Execution Environments (TEEs) are rapidly emerging as a root-of-trust for protecting sensitive applications and data using hardware-backed isolated worlds of execution. TEEs provide robust assurances regarding critical algorithm execution, tamper-resistant credential storage, and platform integrity using remote attestation. However, the challenge of remotely managing credentials between TEEs remains largely unaddressed in existing literature. In this work, we present novel protocols using mutual attestation for supporting four aspects of secure remote credential management with TEEs: backups, updates, migration, and revocation. The proposed protocols are agnostic to the underlying TEE implementation and subjected to formal verification using Scyther, which found no attacks.

==> sections/auditing.tex <==
In IIoT, recording system attributes, such as error details, user activity and potential security events, can underpin audit and after-the-fact forensic investigations, such as if devices bring harm to users like factory floor operatives.   Logs are also used to enforce user accountability, event reconstruction and intrusion detection, and are routinely targeted by attackers to conceal wrongdoing.  Securely storing system logs, as recommended by NIST~\cite{nist:logs} and ISO 27001:2013~\cite{iso}, is hence vital in maintaining its auditability.   NIST SP 800-82 states that an ICS must \emph{``monitor, log, and audit activities occurring on systems and networks...[for] understanding the current state of the ICS, validating that the system is operating as intended, and that no policy violations or cyber incidents have hindered the operation of the system. %Network security monitoring is valuable to characterize the normal state of the ICS, and can provide indications of compromised systems when signature-based technologies fail. 
Additionally, strong system monitoring, logging, and auditing is necessary to troubleshoot and perform any necessary forensic analysis''}~\cite{nist}.  There is little reason why IIoT devices would be excluded if they influence either human or machine operations.

%https://nvd.nist.gov/800-53/Rev4/control/AU-9
NIST SP 800-82~\cite{nist} states little in implementing ICS audit log preservation; however, the NIST SP 800-53~\cite{force} control enhancements suggest, firstly, using Write-Once, Read-Many (WORM) storage, e.g. CD-Rs, for preventing log tampering.  Unfortunately, WORMs are inappropriate for IoT devices without room to accommodate CD-R drives, or necessitating specialist hardware like SD cards that prevent block rewrites (see the SanDisk WORM\footnote{SanDisk WORM: https://goo.gl/f5RYXX}).  Beside this, the guidance suggests \emph{``cryptographic mechanisms to protect the integrity of audit information''}.  Next, we briefly examine the state-of-the-art for cryptographically preserving audit logs using TEEs and TPMs.





%\subsection{Related Work}


%The information system implements cryptographic mechanisms to protect the integrity of audit information and audit tools.
%he  information system  writes  audit  trails to  hardware- enforced, write-once media

Log integrity is commonly preserved using \emph{hash chains}, where a protected record, $\ell_{i}$, is formed by hashing the current record under the hash of the previous, i.e. $\ell_{i} = h(m_{i} || \ell_{i-1})$.  In early work, Schneier and Kelsey~\cite{schneier} form tamper-resistant records comprising: 1), the event message, $m_i$; 2), the current hash chain entry, $\ell_{i} = h(m_{i} || \ell_{i-1})$ where $\ell_0 = h(m_0)$; and 3), a MAC, $Z_i = MAC_{A_i}(\ell_i)$, where $A_i = h(A_{i-1})$ and $A_0$ is a PSK between the device and a third-party verifier.

Such schemes, however, rely on the assumption that the PSK is, indeed, stored securely, and that the retrieval process is trusted.   In recent work~\cite{shepherd:wistp,sinha:tpm,bock,karande}, TPMs and TEEs have been proposed for assuring that logging keys are stored securely, performing cryptographic operations, and providing platform integrity evidence to remote verifiers using remote attestation.    

Sinha et al.~\cite{sinha:tpm} propose using a TPM alongside a forward integrity scheme based on branched key chaining.  Records are divided into epochs (blocks) comprising sequences of hash-chained log entries (sub-epochs).  The root entries of each epoch are hash-chained with past epochs to create a two-dimensional hash chain to prevent \emph{re-ordering attacks} where an attacker re-orders log blocks to mislead auditors.  For a new epoch, the previous epoch's logs are securely stored using the TPM's seal functionality using the TPM's SRK.

B{\"o}ck et al.~\cite{bock} propose AMD's Secure Virtual Machine (SVM) -- a TPM-launched TEE -- for launching a \texttt{syslog} client daemon and logging application.  The logger executes with access to TPM-bound key-pairs for encrypting and signing log entries.  Upon request, the logs are decrypted and released for verification by a third-party; the keys are certified by the TPM vendor to provide assurance that logs were processed in an authentic execution environment.  



%Nguyen et al.~\cite{cloudlogger} propose streaming medical logs to a server application that applies tamper-resistance in Intel SGX (see Section \ref{sec:tees}).  Logs are transmitted to the Intel SGX application (`enclave') over TLS, before computing a hash chain that includes a signature of each record.  A TPM is used to authentication the server to medical devices and to securely store log hash chains using the TPM's sealing mechanism.
% an extension to the Intel architecture that provides integrity and confidentiality assurances to sensitive applications in execution 
Karande et al.~\cite{karande} introduce SGX-Log for protecting logs received from remote devices.  Similar to \cite{sinha:tpm}, SGX-Log constructs block-based hash chains in an Intel SGX enclave to preserve log integrity and confidentiality at run-time.  The authors note that power-loss resilience, where logs in volatile memory are lost due to a power loss, can be provided by continually sealing blocks to file.  The proposal is evaluated using three datasets with a slight ($\sim$7\%) run-time overhead versus a non-SGX implementation.


For constrained devices, Shepherd et al.~\cite{shepherd:wistp} propose EmLog for device-side logs using block-based hash chains and the GP TEE with ARM TrustZone.  It also offers public verifiability of log origin by appending ECDSA signatures to blocks from a TEE-bound key; a trusted path with I/O peripherals, provided natively by TrustZone; and secure block key derivation for bounding the impact of key leakages.  EmLog is evaluated using a Huawei ARM development board with TrustZone and a GP-compliant TEE, with low run-time overhead and five-times storage overhead versus raw logs.
%Numerous proposals suggest using IoT devices for remote health monitoring~\cite{patel}, identifying fires and gas leakages~\cite{chen:home}, and detecting falls and injuries in the homes of the elderly and disabled~\cite{rashidi} -- all of which are natural applications for tamper-resistant logging.  Unfortunately, discrete hardware TPMs, which underpin many existing proposals, cannot directly host arbitrary applications without additional processes, such as launching and locally attesting applications from a TPM-backed virtual machine~\cite{bock,perez2006vtpm}.  Including such processes within the device's Trusted Computing Base (TCB) -- the set of software and hardware components essential to its security -- widens the scope for introducing security and performance defects~\cite{mccune,singareducing}.  One promising solution is the Trusted Execution Environment (TEE), which offers TPM-like functionality alongside strong isolated execution of critical applications, while using the core execution hardware of conventional operating systems.  TEEs have become widely-deployed in recent years, notably in the form of Intel Software Guard eXtensions (SGX) and TEEs built on ARM TrustZone.  Indeed, Trustonic estimated that one billion devices contained their TrustZone-based TEE alone in early 2017~\cite{trustonic}.  However, TEE-based logging schemes -- discussed in Section \ref{sec:related} -- have hitherto applied only server-side TEEs to protect logs transmitted from remote devices.


%\subsection{Proposed Log Transmission Protocol}

\begin{figure}[t]
\includegraphics[width=\linewidth]{./figures/audit.pdf}
\caption{Proposed High-Level Audit Record Transmission Procedure.}
\label{fig:audit}
\end{figure}

While a wealth of literature exists for producing tamper-resistance records, little research exists regarding their secure transmission.  Most schemes, e.g. \cite{bock} and \cite{sinha:tpm}, stipulate the use of a secure channel, such as TLS, while \cite{karande} and \cite{shepherd:wistp} propose one-way and mutual remote attestation channels respectively.  In this work, we propose a log transmission protocol for in IIoT applications.
The proposed transmission procedure is shown in Figure~\ref{fig:audit}.   Structurally, it is virtually identical to the Remote Backup procedure described in Section~\ref{sec:backup} and Figure~\ref{fig:backup}, except the role of the Backup Authority (BA) is replaced with an Auditing Authority (AA).  We refer the reader to Section~\ref{sec:backupprotocol} for a review of this procedure.



%The subsequent audit operations are unprivileged operations; i.e. any Actor, whether authenticated or not,
%may invoke the command that performs the audit operation to retrieve the expected information.
%These audit commands can be submitted to:
% The TMF audit SD (as mentioned in section 4.5) regardless of the TEE life cycle %state
%o This audit SD is identified on the TEE by a reserved UUID value defined in %section A.3.
% Any accessible SD (i.e. not in the Blocked life cycle state) provided that the %TEE is in the
%TEE_SECURED life cycle state
% Any accessible SD (i.e. not in the Blocked life cycle state) with the %gpd.privilege.teeManagement
%privilege when the TEE is in the TEE_LOCKED life cycle state
%%If an audit operation command is submitted with an Authorization Token, the procedure described in
%section 6.1.2 for unprivileged operations SHALL apply before performing any %operation-specific action listed
%in the following

%4.5 TEE Audit Information
%When installing applications on a device that has both an insecure and a secure %side, it is necessary to
%determine information about the capabilities of the TEE into which the secure part %will be installed.
%This information allows an unprivileged application installed in the REE to %determine whether its secure
%component can run and to determine which Authority it should either request %authorization to install its trusted
%component from or request to perform the secure installation. This is especially %important for applications
%which can continue to operate in a degraded manner when their trusted component is %not installed.
%This information is provided in the form of TLV data which is associated with, and %maintained along with, the
%TEE/Trusted OS.
%This specification provides a full description of unprivileged operations allowing %Client Applications to access
%TEE, Security Domain, and Trusted Application characteristics.
%Information returned by the audit functions is in plain text. It SHOULD therefore %be accessed over a channel
%that prevents third parties from modifying the response.
%The audit commands (see section 8.8) corresponding to these unprivileged operations %(see section 6.6) are
%the following:
% Get TEE Definition (section 6.6.1)
% Provides TEE information in TLV format (as defined by section 9.1)
% Get SD Definition (section 6.6.2)
% Provides Security Domain information in TLV format (as defined by section 9.2)
% Get List of Trusted Applications (section 6.6.3)
% Provides the UUIDs of Trusted Applications of a Security Domain
% Get Trusted Application Definition (section 6.6.4)
% Provides Trusted Application information in TLV format (as defined by section 9.3)
%Any audit commands can be submitted to SD-P, where SD-P can be:
% Any Security Domain that is accessible; i.e.:
% The SD is not blocked (Blocked life cycle state) and, if the TEE is locked, the SD %has the
%gpd.privilege.teeManagement privilege.
% The audit SD defined by this specification (hereafter called the TMF audit SD):
% Its reserved UUID is defined in section A.3.
% It is capable of performing only unprivileged audit operations. Any attempt to use %it to perform
%any other administration command will be rejected with the TEE_ERROR_DENIED_ACCESS
%error code.
% It is implementation-defined whether the TMF audit SD is made available to Trusted
%Applications executing within the TEE.
